Long-tail Detection with Effective Class-Margins

Large-scale object detection and instance segmentation face a severe data imbalance. The finer-grained object classes become, the less frequent they appear in our datasets. However, at test-time, we expect a detector that performs well for all classes and not just the most frequent ones. In this paper, we provide a theoretical understanding of the long-trail detection problem. We show how the commonly used mean average precision evaluation metric on an unknown test set is bound by a margin-based binary classification error on a long-tailed object detection training set. We optimize margin-based binary classification error with a novel surrogate objective called \textbf{Effective Class-Margin Loss} (ECM). The ECM loss is simple, theoretically well-motivated, and outperforms other heuristic counterparts on LVIS v1 benchmark over a wide range of architecture and detectors. Code is available at \url{https://github.com/janghyuncho/ECM-Loss}.

==> intro.tex <==
\section{Introduction}

\label{sec:intro}

Object detection is a core computer vision task and has seen a great success in recent years. Notably, the state-of-the-art performance of common object detectors has more than tripled over the past 5 years, on the popular COCO dataset benchmark~\cite{coco}. However, such dataset contains far less number of object categories (80 in COCO) compared to the real-world data, and the data distribution is highly curated to balance over the categories. With large number of object categories, labeling cost will grow substantially and maintaining balanced data distribution is not only expensive but also infeasible in the real-world scenarios; labeling more images will uncover previously unseen rare categories and maintain the long tail~\cite{lvis}. Hence, facing data imbalance problem is an essential step towards large-scale, general-purpose object detector. 

% In object detection, data imbalance problem is in two-folds: cross-category imbalance and foreground-background imbalance. For small-scale data with absence of cross-category imbalance, foreground-background imbalance problem has been addressed by cascading via RPN~\cite{fasterrcnn} and sampling heuristics in two-stage detectors, and by heuristically shaped learning objectives such as Focal Loss~\cite{focal}. 


To account the scaling trend of modern object detector, a number of large-scale object detection dataset has been released~\cite{lvis,openimages,o365}. In particular, LVIS dataset contains instance segmentation labels of 1203 object categories that are collected in federated manner. This dataset reflects realistic issues of the real-world such as extreme long-tailed data distribution and non-exhaustive annotations. Especially such extreme imbalance in data distribution makes training an object detector challenging in several ways. First, classes in low-data regime will undergo extremely large frequency of update with negative samples, which leads to a biased model prediction during evaluation where each class is considered equally important. Furthermore, the learning objective faces imbalance between foreground and background even without the inter-class data imbalance, yet the background class is only to reduce the false positive of predictions, not to be evaluated explicitly. This adds another layer of complication to the problem, causing many successful methods for classification~\cite{ldam, cb_focal, ncm} under imbalanced distribution underperform compared to simple baselines~\cite{focal}. In sum, the evaluation metric for object detection is average precision (AP) which implicitly involves ranking among predictions through precision and recall, and it is unclear how to handle such imbalance with loss functions that are designed based on classification error (i.e., zero-one error). 


There has been a number of successful approaches to solve the long-tailed object detection task. A large body of works~\cite{seesaw, federated_loss, eqlv1, eqlv2, bags} focus on the premise that reducing the amount of negative gradients on rare classes will translate to better performance overall. These methods have their own strategies to control the negative gradients on the rare classes, either explicitly or implicitly. However, despite their success, these methods are hardly justified and often exhaustively engineered with heuristics with less intuition. This makes further research particularly challenging and may lead to suboptimal solutions. 

In this paper, we take a step towards answering how to approach to the problem and optimize in the perspective of generalization error bound~\cite{lipschitz, barlett, ldam}. We first draws connection between the exact object detection metric (AP) to binary classification, and refer to the large body of theoretical studies in margin theory. We motivate from the observation that many of the recently successful methods can be reformulated to soft-margin cross-entropy loss with different choices of margins for each class, the relationship between margins to impose during training and the model's ability to generalize can give us a hint to optimize the margins to improve the detector's performance during evaluation. Hence, we propose a simple, theoretically justified strategies of effective class-margin assignment, through our Effective Class-Margin Loss (ECM Loss). Object detector trained with ECM Loss on large-scale datasets such as LVIS and OpenImages outperforms many recent methods including the state-of-the-art by large margin, on various choice of frameworks, backbone, and other settings. 


% \subsection{Sketch}
% \begin{enumerate}
%     \item \sout{Common object detection performance does not reflect the large-scale data distribution. }
%     \item \sout{Learning from large-scale data faces severe imbalance issues. }
%     \item \sout{Imbalance in detection is deeply complicated with foreground background imbalance and foreground imbalance.} 
%     \item \sout{Previously, with small dataset, either RPN or Focal Loss is used to address the issue. }
%     \item In imbalanced classification, margin theory-based losses are used. 
%     \item In large-scale detection, these two problems are deeply intertwined in the following reasons. 
%     \item 1. Evaluation objective is not classification error but a form of ranking error (AP).
%     \item 2. The categories of interest are foreground only; background implicitly influence the performance. 
%     \item 3. For each class, the positive and negative are a mixture of other foregrounds and background.
%     \item For these reasons, traditional margin-based learning objective tend to fail in object detection. 
%     \item successful detection losses require heuristic engineering efforts and not intuitive. 
%     \item The direction to face the problem is from the evaluation metric: what do we care and how is it linked in learning process? 
% \end{enumerate}







% To account the scaling trend of modern visual system, a number of large-scale object detection dataset has been released~\cite{lvis,openimages,o365}. In particular, LVIS dataset contains instance segmentation labels of 1203 object categories that are collected in federated manner. This dataset reflects realistic issues of the real-world such as extreme long-tailed data distribution and non-exhaustive annotations. 






% Especially such extreme imbalance in data distribution makes training an object detector challenging in several ways. First, classes in low-data regime will undergo extremely large frequency of ``negative gradient updates,'' which leads to biased model prediction during evaluation where each class is considered equally important. Furthermore, by the nature of object detection process, the learning objective faces imbalance between foreground and background even without the aforementioned data imbalance, yet the background class is only to reduce the false positive of predictions, not to be evaluated explicitly. This adds another layer of complication to the problem, causing many successful methods for classification~\cite{ldam, cb_focal, ncm} under imbalanced distribution underperform compared to simple baselines~\cite{focal}. 



% There has been many successful approaches to solve the long-tailed object detection task specifically. A large body of works~\cite{seesaw, federated_loss, eqlv1, eqlv2, bags} focus on the premise that \emph{reducing the amount of negative gradients will translate to better performance overall}. These methods have their own strategies to control the negative gradients on the rare classes, either explicitly or implicitly. However, despite their success, these strategies are hardly justified and often exhaustively engineered with heuristics. This makes further research particularly challenging and may lead to suboptimal solutions. 


% In this paper, we take a step towards answering \emph{why} these strategies work, and \emph{how} to improve in the perspective of generalization error bound. We motivate from the observation that many of the recently successful methods can be reformulated to soft-margin cross-entropy loss, with different choices of margins for each class. The theoretical studies of relationship between margins to impose during training and the model's ability to generalize can give us a hint to optimize those margins to improve the model's performance during evaluation. Hence, we propose a simplistic, theoretically justified strategies of effective class-margin assignment, through our Effective Class-Margin Loss. Object detector trained with ECM Loss on the large-scale datasets outperforms many recent methods including the state-of-the-art by large margin, on various choice of frameworks, backbone, and other settings. 

==> main_table.tex <==
\begin{table*}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccccc}
Framework & Backbone & Sampler  & Schedule & Method & mAP_{\text{segm}} & AP_\text{r} & AP_\text{c}& AP_\text{f} & mAP_{\text{bbox}}\\
\toprule
\multirow{4}{*}{Mask R-CNN}&
\multirow{4}{*}{ResNet-50}&\multirow{4}{*}{RFS} & \multirow{4}{*}{2x} & CE Loss & 22.7 & 10.6 & 21.8 & 29.1 & 23.3\\
& & && Federated Loss & 26.0 & 18.7 & 24.8 & 30.6 & 26.7  \\
& & && Seesaw Loss & 26.7 & 18.0 & 26.5 & 32.4 & 27.3\\
& & && \ours  & 27.4 & 19.7 &27.0&31.1 & 27.9 \\
\midrule
\multirow{6}{*}{Mask R-CNN}&
\multirow{6}{*}{ResNet-101}&\multirow{6}{*}{RFS} & \multirow{6}{*}{2x} & CE Loss & 25.5 & 16.6 & 24.5 & 30.6 & 26.6\\
& & && EQL v1& 26.2 & 17.0 & 26.2 & 30.2  & 27.6 \\ 
& & && BAGS &  25.8 & 16.5 & 25.7 & 30.1 & 26.5\\
& & && Federated Loss & 27.9 & 20.9 & 26.8 & 32.3 & 28.8  \\
& & && Seesaw Loss &28.1 & 20.0 & 28.0 & 31.8 & 28.9\\
& & && \ours & \\
\midrule
\multirow{6}{*}{Cascade Mask R-CNN}&
\multirow{6}{*}{ResNet-101}&\multirow{6}{*}{RFS} & \multirow{6}{*}{2x} & CE Loss  & 27.0 & 16.6 & 26.7 & 32.0 & 30.3\\
& & && EQL v1 &  27.1 & 17.0 & 27.2 & 31.4 & 30.4 \\ 
& & && BAGS & 27.0 & 16.9 & 26.9 & 31.7  & 30.2\\
& & && Federated Loss & 28.6 & 20.3 & 27.5 & 33.4 & 31.8 \\
& & && Seesaw Loss & 30.1 & 21.4 & 30.0 & 33.9 & 32.8\\
& & && \ours &  \\
\midrule
\multirow{3}{*}{Cascade Mask R-CNN}&
\multirow{3}{*}{Swin-B}&\multirow{3}{*}{RFS} & \multirow{3}{*}{2x} & Seesaw Loss  & 38.7 & 34.3 & 39.6 & 39.6 & 42.8 \\
& & && Federated Loss &  &\\
& & && \ours & \\
\bottomrule
\end{tabular}
}
\end{center}
\vspace{-2mm}
\caption{Main table for 2-stage frameworks on LVIS-v1 benchmark. }
\label{tab:main_table}
\vspace{-6mm}
\end{table*}


==> method.tex <==

\section{Effective Class Margins}
\label{method}

In this section, we relate AP, R, and classification. This allows us to apply margin-based generalization bound which leads to derive effective class margins for learning from long-tail data following~\cite{ldam}. 

\subsection{Connection from AP to R}
We first show that AP can be bounded from above and below by R as following.
\begin{theorem}[R upper-bound]
\label{r_upper}
\begin{align}
\ap_c \le 1 - \frac{\alpha_c}{1+\alpha_c}\pr_c 
\end{align}
\begin{proof}
% The complete proof will be in supplementary.
From our definition of precision:
\begin{align}
\pre_c(t) 
&= \frac{P_{x\sim \pc}(\f(x)_ c > t)}{P_{x\sim  \pc}(\sig > t) + \alpha_c  P_{x \sim  \pnc}(\sig > t)} \\
&= 1- \frac{\alpha_c  P_{x \sim  \pnc}(\sig > t)}{P_{x\sim  \pc}(\sig > t) + \alpha_c  P_{x \sim  \pnc}(\sig > t)} \\
&\le 1- \frac{\alpha_c }{1+\alpha_c} P_{x \sim  \pnc}(\sig > t)
\end{align}
Now, by Theorem~\ref{ap_alternative} and Theorem~\ref{r_alternative}:
\begin{align}
\ap_c &= \e_{t\sim P_{s_c^+}}[\pre(t)]\\
&\le 1 - \frac{\alpha_c}{1+\alpha_c}\e_{t \sim P_{s^+_c}}\Big[P_{x \sim  \pnc}(\sig > t)\Big]\\
&=1 - \frac{\alpha_c}{1+\alpha_c}\pr_c
\end{align}
\end{proof}
\end{theorem}

\begin{theorem}[R lower-bound]
\label{r_lower}
\begin{align}
\ap_c \ge \max \bigg(1 - \sqrt{\frac{2}{3}\alpha_c \pr_c}, \frac{8}{9} \frac{1}{1+2 \alpha_c \pr_c}\bigg)
\end{align}
\begin{proof}
The complete proof will be in supplementary.
\end{proof}
\end{theorem}


\begin{lemma}[Linear approximation]
\label{linear_approx}
We can approximate the relation between 1-AP and R with a linear line intersecting the two points where the upper and lower bounds meet:
\begin{align}
\text{det}_c=1-\ap_c  \le w_c\pr_c  
\end{align}
for some $w_c$ for each class $c\in \y$. 
\begin{proof}
\begin{align}
\text{lower}(r) &= \max\bigg(1 - \sqrt{\frac{2}{3}\alpha r}, \frac{8}{9} \frac{1}{1+2 \alpha r}\bigg)\\
\text{upper}(r) &= 1 - \frac{\alpha_c}{1+\alpha_c}(1-\pr_c)
\end{align}
$\text{lower}(r)$ and $\text{upper}(r)$ meets at $r=0$, and a point $r \in [0, 1]$. Solving for r:
\begin{align}
&\max\bigg(1 - \sqrt{\frac{2}{3}\alpha r}, \frac{8}{9} \frac{1}{1+2 \alpha r}\bigg) = 1 - \frac{\alpha}{1+\alpha}(1-r)\\
 &r = \frac{-9 + \sqrt{73 + 64\alpha}}{6\alpha}\\
&\ap \ge\bigg( \frac{8}{-18 + 3\sqrt{73+64\alpha}}-1\bigg)\pr
\end{align}
\end{proof}
\end{lemma}

We can also upper-bound PR by classification as following.
\begin{theorem}[Binary upper bound]
\label{binary_upper}
\begin{align}
\pr_c
&\le \p_{x \sim \pc}\big(\f(x)_c \le \gamma_c  \big) + \p_{x\sim \pnc}\big(\f(x)_{\lnot c} \le \gamma_{\lnot c} \big)
\end{align}
for any $\gamma_c, \gamma_{\lnot c} > 0$, where $\f(x)_{\lnot c} =- f(x)_c$. 
% \begin{proof}
% The complete proof will be in supplementary. 
% \end{proof}
\end{theorem}
Putting all-together, we have the following connection from AP to classification.
\begin{theorem}[Detection bound]
\label{detbound}
Combining Lemma~\ref{linear_approx} and Theorem~\ref{binary_upper}: 
\begin{align}
\text{det}_c&\overset{\Delta}{=}1-AP_c\\ 
&\le w_c\Big(\p_{x \sim \pc}\big(\sig \le 1/2 + \gamma_c \big)+\p_{x\sim \pnc}\big(1-\sig \le 1/2 - \gamma_c\big)\Big)
\end{align}
where $\det_c$ is detection error of a class $c$. 
\end{theorem}

Let us start from our pairwise-ranking error. 
\begin{align}
R_c 
&= P_{x^+\sim P_c, x^-\sim P_{\lnot c}}(\sigma(f_\theta(x^+))_c \le \sigma(f_\theta(x^-))_c)\\
&\le P_{x^+\sim P_c}(\sigma(f_\theta(x^+))_c \le t) +  P_{x^-\sim P_{\lnot c}}(\sigma(f_\theta(x^-))_c > t)
\end{align}
where $\sigma$ is a sigmoid function, and for any $t \in \mathbb{R}$. Let us set $t=\frac{1}{2}+\gamma_c$ where $\gamma_c > 0$. Notice when $t=1/2$, the above reduces to a regular binary classification. This allows us to enforce non-negative class-margin $\gamma_c$ which we will later optimize for. Then, 
\begin{align}
R_c 
&\le P_{x^+\sim P_c}(\sigma(f_\theta(x^+))_c \le 1/2+\gamma_c) +  P_{x^-\sim P_{\lnot c}}(\sigma(f_\theta(x^-))_c > 1/2+\gamma_c)\\
&=P_{x^+\sim P_c}(\sigma(f_\theta(x^+))_c \le 1/2+\gamma_c) +  P_{x^-\sim P_{\lnot c}}(1-\sigma(f_\theta(x^-))_c \le 1/2-\gamma_c)\\
\Longrightarrow \text{det}_c &= 1-AP_c \le w_c R_c \\
&\le  w_c\Big(\p_{x \sim \pc}\big(\sig \le 1/2 + \gamma_c \big)+\p_{x\sim \pnc}\big(1-\sig \le 1/2 - \gamma_c\big)\Big)
\end{align}
The above inequality states that ``detection error is upper-bounded by binary classification errors from two distributions $P_c$ and $P_{\lnot c}$.  Let us recap the Lipschitz-based generalization bound for binary classification error from Barlett and Mendelson~\cite{bartlett}.
\begin{theorem}[Lipschitz bound]
\label{lipschitz}
Assume the loss $\ell$ is Lipschitz (with respect to its first argument) with Lipschitz constant L and that $\ell$ is bounded by $c$. For any $\delta > 0$ and with probability at leats $1-\delta $ simultaneously for all $f \in \mathcal{F}$, we have that
\begin{align}
\mathcal{L}(f) \le \hat{\mathcal{L}}(f) + 2L \mathcal{R}_n(\mathcal{F}) + c \sqrt{\frac{\log(1/\delta)}{2n}}
\end{align}
where $\mathcal{R}_n(\mathcal{F})$ is the Rademacher complexity of a function class $\mathcal{F}$, and $n$ is the sample size. 
\end{theorem}
One special case of Theorem~\ref{lipschitz} is the following margin bound:
\begin{theorem}[Margin bound]
Consider an arbitrary function class $\mathcal{F}$ such that $\forall f \in \mathcal{F}$, we have $\sup_{x\in \mathcal{X}} |f(x)| \le M$. And the zero-one loss function is given by $\ell (f(x),y)=\mathrm{I} [f(x)_y < 0]$ , and the $\gamma$-margin zero-one loss function is given by $\ell_\gamma (f(x), y) = \mathrm{I} [ f(x)_y < \gamma]$. Finally, similar to $\mathcal{L}(f)$ and $\hat{\mathcal{L}}(f)$, $\mathcal{L}_\gamma (f) = E [ \ell_\gamma (f(x), y)]$ and $\hat{\mathcal{L}}_\gamma(f) = \frac{1}{n}\sum_{i=1}^n \ell_\gamma (f(x_i), y_i)$.  Then, with probability at least $1-\delta$ over the sample, for all margins $\gamma > 0$ and all $f \in \mathcal{F}$:
\begin{align}
    \mathcal{L}(f) \le \hat{\mathcal{L}}_\gamma (f) + \frac{4}{\gamma} \mathcal{R}_n(\mathcal{F}) + \sqrt{\frac{\log(\log_2 \frac{4M}{\gamma})}{n}} + \sqrt{\frac{\log (1/\delta)}{2n}}
\end{align}
\end{theorem}
Here the classification error is upper-bounded by a Lipschitz continuous \emph{ramp} function $\phi_\gamma$, with constant $\text{Lip}(\phi_\gamma)=\frac{1}{\gamma}$. In fact, the Lipschitz bound is general that one can bound generalization with any Lipschitz continuous error function. Now, consider the following:
\begin{theorem}
Sigmoid function is Lipschitz continuous with constant 1.
\begin{align}
\zeta_c(x) = \sigma(x), \quad \Longrightarrow\quad \text{Lip}(\zeta_c) = 1
\end{align}
for all $c\in \y$, and $x \in \mathbb{R}$. 
\begin{proof}
Lipschitz constant $m$ of a function $\zeta:\mathbb{R}\rightarrow \mathbb{R}$ is defined as following:
\begin{align} 
|\zeta(x) - \zeta(y)| \le m\cdot | x-y|
\end{align}
Starting from the left hand side:
\begin{align}
|\zeta(x) - \zeta(y)| 
&= |\vec{\nabla \zeta(z)}^\top (x-y)|\\
&\le |t \nabla \zeta(z)|\cdot | x-y|
\end{align}
due to Mean-Value Theorem for some $z$ and Cauchy-Schwarz inequality. Then,
\begin{align}
\vec{\nabla \zeta_c(z)} = \begin{cases}
\sigma(z)_c \cdot \sigma(z)_i & \text{if} \quad i\ne c\\
\sigma(z)_c \cdot (\sigma(z)_i - 1) & \text{if} \quad i=c
\end{cases}
\end{align}
where $|\vec{\nabla \zeta_c(z)}|$ is bounded by 1. Therefore, 
\begin{align}
\text{Lip}(\zeta_c) =1 \quad \forall c\in \y
\end{align}
\end{proof}
\end{theorem} 
Our error function is a composite function of a standard zero-one error and sigmoid function, which is equivalent to having a new error function $\eta = \zeta \circ \phi_\gamma$. 
\begin{lemma}
For $\eta=\zeta \circ \phi_\gamma$:
\begin{align}
\text{Lip}(\eta) = \frac{1}{\gamma}
\end{align}
\begin{proof}
\begin{align}
|\eta(x)-\eta(y)| &= |\phi_\gamma(\zeta(x))-\phi_\gamma(\zeta(y))|\\
&\le \frac{1}{\gamma}|\zeta(x)-\zeta(y)|\\
&\le \frac{1}{\gamma}\Vert x-y\Vert
\end{align}
\end{proof}
\end{lemma}
Let us define the set of data sampled from $P_c$ and $P_{\lnot c}$ be $S_c$ and $S_{\lnot c}$. Putting all-together, we have the following upper-bound to the detection error:
\begin{align}
\text{det}_c \le w_c \Bigg(&\frac{1}{n^+_c}\sum_{x^+\in S_c}\mathbb{I}\{\sigma(f_\theta(x^+))_c \le 1/2+\gamma_c\}\\
+ &\frac{1}{n^-_c}\sum_{x^-\in S_{\lnot c}}\mathbb{I}\{1-\sigma(f_\theta(x^-))_c \le 1/2-\gamma_c\}\\
+ &\frac{4}{1/2+\gamma_c}\sqrt{\frac{C(\Theta)}{n^+_c}} + \frac{4}{1/2-\gamma_c}\sqrt{\frac{C(\Theta)}{n^-_c}} + \epsilon(n^+_c) + \epsilon(n^-_c)\Bigg)
\end{align}
With separability assumption, we can derive the optimal margin $\gamma_c$ for each class separately: 
\begin{align}
\gamma_c 
&= \arg\min_\gamma \frac{4}{1/2+\gamma_c}\sqrt{\frac{C(\Theta)}{n^+_c}} + \frac{4}{1/2-\gamma_c}\sqrt{\frac{C(\Theta)}{n^-_c}} \\
&= \arg\min_\gamma \frac{1}{1/2+\gamma_c}\sqrt{\frac{1}{n^+_c}} + \frac{1}{1/2-\gamma_c}\sqrt{\frac{1}{n^-_c}} \\
 &= \Bigg| \frac{1}{2} \frac{(n^+_c)^{1/4} - (n^-_c)^{1/4}}{(n^+_c)^{1/4}+(n^-_c)^{1/4}} \Bigg|\quad \text{for feasible } \gamma_c
\end{align}


\subsection{ECM Loss}
Now, let us derive our surrogate loss. Starting from empirical 0-1:
\begin{align}
\hat{l}^+_c(x,y)
&= \mathbb{I}\{\sigma(f_\theta(x))_c \le 1/2+\gamma_c\}\\
&= \mathbb{I}\{\log (\sigma(f_\theta(x))_c) \le \log ( 1/2+\gamma_c)\}\\
&= \mathbb{I}\Big\{-\log\Big(\underbrace{(1/2+\gamma_c)^{-1}}_{=w^+_c}\cdot \sigma(f_\theta(x))_c\Big) > 0 \Big\}\\
\hat{l}^-_c(x,y)
&= \mathbb{I}\{1-\sigma(f_\theta(x))_c \le 1/2-\gamma_c\}\\
&= \mathbb{I}\{\log( 1-\sigma(f_\theta(x))_c) \le \log ( 1/2-\gamma_c)\}\\
&= \mathbb{I}\Big\{-\log\Big(\underbrace{(1/2-\gamma_c)^{-1}}_{=w^-_c}\cdot (1-\sigma(f_\theta(x))_c)\Big) > 0 \Big\}
\end{align}

For both error terms, we want to minimize the LHS inside the indicator function. Hence we define our surrogate loss to be the following:
\begin{align}
l_{sur}(x,y) = - \Big(\log (w^+_c\cdot \sigma_c) + \log (w^-_c\cdot(1-\sigma_c))\Big)
\end{align}
which is a binary cross-entropy loss with scaled confidences. One issue with the above formulation is that the weights can be arbitrarily large, and make the loss to be negative. Therefore, we normalize the confidence term with the weights as the following:
\begin{align}
{w_y}^+\cdot \sigma(x) &= \frac{{w_y}^+ \cdot e^x}{e^x + e^{-x}} \in \mathbb{R}_+\\
\Longrightarrow \sigma_{w_y}(x) &= \frac{{w_y}^+ \cdot e^x}{{w_y}^+\cdot e^x + {w_y}^-\cdot e^{-x}}\in [0, 1]
\end{align}
which is bounded by 1, proper to be a valid probability estimation. Finally, we have
\begin{align}
l_{w_y}(x,y) = - \Big(\log (\sigma_{w_y}(f_\theta(x)_y) + \log (1-\sigma_{w_y}(f_\theta(x)_y) \Big)
\end{align}
which is a binary cross-entropy loss with weighted sigmoid function, named \emph{Effective Class-Margin Loss}.



==> prelim_v2.tex <==
\section{Preliminary}
In object detection, the performance of a model is measured by average precision (AP) over different values of recall. Precision and recall are defined with the count of true positive, false positive, and false negative of a model's prediction with respect to a confidence threshold $t$:
\begin{align}
    % TP_c(t) &= |\{s(x)_c > t: x,y \in S\}|\\
    % FP_c(t) &= |\{s(x)_c > t: x,y \in S\}|\\
    % FN_c(t) &= |\{s(x)_c < t: x,y \in S\}|\\
    p(t)&=\frac{TP(t)}{TP(t) + FP(t)}\quad r(t) = \frac{TP(t)}{TP(t) + FN(t)}\quad AP= \frac{1}{|T|} \sum_{t\in T}p(t)
\end{align}
where $T$ is a set of thresholds $t$ such that $r(t)$ evenly covers $[0,1]$. To design a learning objective for object detector under data-imbalanced setting, a natural question to ask is how to maximize test AP, or equivalently, minimize the test detection error $\ldet=1-AP$. Motivated from classification literature with zero-one error~\cite{ldam, bartlett, kakade}, we can formulate the generalization error in terms of true and empirical detection errors $\ldet$ and $\lhdet$:
\begin{align}
    \text{Generalization Error} \overset{\Delta}{=} \mathcal{L}_{\text{Det}} - \hat{\mathcal{L}}_{\text{Det}} 
\end{align}
When considering \textit{separable} case, bounding the generalization error in terms of controllable factors such as\textit{ class margins } allow us design a learning objective more strategically. However, it is 1) unclear how to properly define the generalization error with respect to detection error, since AP is defined entirely in empirical manner. Moreover, unlike classification error, detection error is much more complex, depends not only on the data distribution but also on the distribution of the model's confidence. Hence, 2) bounding the detection error with simple class margins is challenging. In this paper, we will answer these questions. Please find all missing proofs in the supplementary. 
\subsection{Probabilistic Interpretations}
Let us properly define the detection error $\ldet$. With infinitely many samples drawn from data distribution, each definition of detection metrics falls into the following probabilistic interpretations for each class $c\in C$.
\begin{definition}[Probabilistic Precision, Recall, and AP]
\begin{align}
p_c( t) 
&= \underbrace{P_{x, y \sim P(X,Y)}(y=c|\sig > t)}_{\text{``true given positive''}}= \frac{P_{x\sim \pc}(\sig > t)}{P_{x\sim  \pc}(\sig > t) + \alpha_c  P_{x \sim  \pnc}(\sig > t)}\\
r_c( t) &= \underbrace{P_{x,y \sim P(X,Y)}(\sig > t | y=c)}_{\text{``positive given true''}}=P_{x\sim  \pc}(\sig > t)\\
\ap_c 
&=\underbrace{ \int^1_0 \pre_c (\rec_c(\beta)^{-1})\mathrm{d}\beta}_{\text{``precision at recalls over [0,1]''}} =  \e_{t\sim P_{s_c}}[\pre_c(t)]
\end{align}
\end{definition}
where $\alpha_c = \frac{P(y\ne c)}{P(y= c)}$. 
% The above definitions allow us to properly formulate the gap between true detection error and sample detection error. However, 
AP is intertwined with model's confidence and data distribution over samples, infeasible to construct a simple learning objective (i.e., surrogate loss) with its current form. From below, we decouple the model's confidence and the data distribution from the metric. First, consider the following new, related metric called \emph{Pairwise Ranking Error}: 
\begin{definition}[Pairwise Ranking Error]
\begin{align}
\pr_c 
&= \p_{x, x' \sim \pc \times \pnc} \big(\sigp < \sigm \big)\\
&= \e_{t \sim P_{s_c}}\Big[P_{x \sim  \pnc}\big(\sig > t\big)\Big]
\end{align}
\end{definition}
Pairwise Ranking Error measures how much a model mis-ranks given a pair of samples from positive and negative distributions. Conveniently, model's confidence is separated from the integration, decoupled from data distributions $\pc$ and $\pnc$. Next, we will connect Pairwise Ranking Error to AP in the form of upper and lower bounds. 
\subsection{Detection Error Bound}
Below, we will show that Pairwise Ranking can be closely related to AP in terms of upper and lower bounds. 
\begin{theorem}[AP - Pairwise Ranking Bound]
\label{r_upper}
\begin{align}
\max \bigg(1 - \sqrt{\frac{2}{3}\alpha_c \pr_c}, \frac{8}{9} \frac{1}{1+2 \alpha_c \pr_c}\bigg) \le \ap_c \le 1 - \frac{\alpha_c}{1+\alpha_c}\pr_c 
\end{align}
\end{theorem}
The above bound allows to approximate the relation between $\ldet$ and $R$ with a linear line intersecting the two points where the upper and lower bounds meet: 
\begin{align}
\mathcal{L}_{\text{Det}}_c \approx w_c\pr_c  \label{linear_approx}
\end{align}
where $w_c=1-\frac{8}{9(1+2\alpha_c)} \Big(\frac{6\alpha_c+3+\sqrt{9(2\alpha_c+1)^2+8(1+\alpha_c))}}{12\alpha_c}\Big)^{-1}$. Moreover, the Pairwise Ranking Error can be upper-bounded by \textit{binary error form} for any arbitrary confidence threshold $t \in [0, 1]$ :
\begin{theorem}[Binary Upper Bound]
\label{r_upper}
\begin{align}
\pr_c &\le \p_{x \sim \pc}\big(\sig \le t\big)+\p_{x\sim \pnc}\big(\sig > t\big)\\
\Longrightarrow \mathcal{L}_{\text{Det}}_c &\lesssim w_c\Big(\p_{x \sim \pc}\big(\sig \le 1/2 + \gamma_c \big)+\p_{x\sim \pnc}\big(1-\sig \le 1/2 - \gamma_c\big)\Big)\label{detection_bound}
\end{align}
\end{theorem}
where $\lesssim$ is a bound up to the approximation in Eqn.~\ref{linear_approx} and for $t=\frac{1}{2}+\gamma_c$. Notice that with $\gamma_c=0$, the above upper bound boils down to binary classification error. Therefore, by choosing a proper non-negative class margin $\gamma_c$, we can optimize the detection generalization bound.

\section{Effective Class-Margin Loss}
Bounding the generalization error of binary classification in terms of margins usually start with Lipschitz bound from Barlett and Mendelson~\cite{lipschitz}.
\begin{theorem}[Lipschitz bound~\cite{lipschitz}]
\label{lipschitz}
Assume the loss $\ell$ is Lipschitz (with respect to its first argument) with Lipschitz constant L and that $\ell$ is bounded by $c$. For any $\delta > 0$ and with probability at leats $1-\delta $ simultaneously for all $f \in \mathcal{F}$, we have that
\begin{align}
\mathcal{L}(f) \le \hat{\mathcal{L}}(f) + 2L \mathcal{R}_n(\mathcal{F}) + c \sqrt{\frac{\log(1/\delta)}{2n}}
\end{align}
\end{theorem}
where $\mathcal{R}_n(\mathcal{F})$ is the Rademacher complexity of a function class $\mathcal{F}$ which is typically bounded by $\sqrt{\frac{C(\Theta)}{n}}$ for some complexity measure of $C$~\cite{ldam, kakade, bartlett}. A popular margin bound from Kakade et al.~\cite{kakade} extends the Thm.~\ref{lipschitz} for a margin $\gamma$, as zero-one error function with a margin can be extended to a continuous ramp function $\phi_\gamma$ with Lipschitz constant $L=\frac{1}{\gamma}$. We further extend the theorem by simply showing that activation function (i.e., sigmoid) together with zero-one error is Lipschitz continuous, and therefore further upper-bound our detection bound in Eqn.~\ref{detection_bound}.  
\begin{theorem}[Lipschitz Continuity and Detection Bound]
\begin{align}
\mathbb{I}\{s(x) < t\} \le \phi_t(s(x))=\phi_t(\sigma(f_\theta(x))_c) \Longrightarrow \text{Lip}(\sigma\circ \phi_t) = \frac{1}{t}
\end{align}
\end{theorem} 
where the confidence function $s$ is composed of a deep network $f_\theta$ and sigmoid function $\sigma$. Finally, we can directly apply Thm.~\ref{lipschitz} to the detection bound~\ref{detection_bound}.
\begin{align}
\ldet_c \!\lesssim\! w_c \Bigg(\lhdet_c \!+\! \lhdet_{\lnot c}
\!+\! \frac{2}{1/2\!+\!\gamma_c}\sqrt{\frac{C(\Theta)}{n_c}} \!+\! \frac{2}{1/2\!-\!\gamma_c}\sqrt{\frac{C(\Theta)}{n_{\lnot c}}} \!+\! \epsilon(n_c) \!+\! \epsilon(n_{\lnot c})\Bigg)
\end{align}
With separability assumption, we can finally derive the optimal class-margin $\gamma_c$, similar to Cao et al.~\cite{ldam}: 
\begin{align}
\gamma_c 
&= \arg\min_\gamma \frac{2}{1/2\!+\!\gamma_c}\sqrt{\frac{C(\Theta)}{n_c}} \!+\! \frac{2}{1/2\!-\!\gamma_c}\sqrt{\frac{C(\Theta)}{n_{\lnot c}}}\\
&= \frac{1}{2} \frac{(n^+_c)^{1/4} - (n^-_c)^{1/4}}{(n^+_c)^{1/4}+(n^-_c)^{1/4}} \quad \text{for feasible } \gamma_c
\end{align}


\subsection{Surrogate Loss}
Now, let us derive our surrogate loss. Starting from empirical 0-1:
\begin{align}
\hat{l}^+_c(x,y)
&= \mathbb{I}\{s(x)_c \le 1/2+\gamma_c\}\\
&= \mathbb{I}\Big\{-\log\Big(\underbrace{(1/2+\gamma_c)^{-1}}_{=w^+_c}\cdot s(x)_c\Big) > 0 \Big\}\\
\hat{l}^-_c(x,y)
&= \mathbb{I}\{1-s(x)_c \le 1/2-\gamma_c\}\\
&= \mathbb{I}\Big\{-\log\Big(\underbrace{(1/2-\gamma_c)^{-1}}_{=w^-_c}\cdot (1-s(x)_c)\Big) > 0 \Big\}
\end{align}

For both error terms, we want to minimize the LHS inside the zero-one function. Hence, a natural form of the surrogate loss would be the following:
\begin{align}
l_{sur}(x,y) = - \Big(y\cdot \log (w^+_c\cdot s(x)_c) + (1-y)\cdot \log (w^-_c\cdot(1-s(x)_c))\Big)
\end{align}
which is a binary cross-entropy loss with scaled confidences. One issue with the above formulation is that the weights can be arbitrarily large, and make the loss to be negative. Therefore, we normalize the confidence term with the weights as the following:
\begin{align}
{w_y}^+\cdot s(x)_c &= \frac{{w_y}^+ \cdot e^{f_\theta(x)_c}}{e^{f_\theta(x)_c} + e^{-f_\theta(x)_c}} \in \mathbb{R}_+\\
\Longrightarrow s_{w_y}(x)_c &= \frac{{w_y}^+ \cdot e^{f_\theta(x)_c}}{{w_y}^+\cdot e^{f_\theta(x)_c} + {w_y}^-\cdot e^{-f_\theta(x)_c}}\in [0, 1]
\end{align}
which is bounded by 1, proper to be a valid probability estimation. Finally, we have
\begin{align}
l_{\text{ECM}}(x,y) = - \Big(y\cdot \log (s_{w_y}(x)_c) + (1-y)\cdot \log (1-s_{w_y}(x)_c) \Big)
\end{align}
which is a binary cross-entropy loss with weighted sigmoid function, we name \textbf{Effective Class-Margin Loss}.



==> preliminary.tex <==

\section{Preliminary}
\label{preliminary}


In this section, we will discuss preliminary definitions of object detection metrics. We will use notations $\pc = P(x|y=c)$ and $\pnc = P(x|y\ne c)$ that are the class-conditional image distribution of class $c$ (positive distribution) and ``anything but $c$'' (negative distribution), respectively. The model is a function $f\in \mathcal{F}$ with parameters $\theta \in \Theta$. We denote $\f(x)_c$ to be the model prediction (\emph{logit}) and $\sig$ to be the model confidence (\emph{score}) for the class $c\in \y$ from an input $x \in \mathcal{X}$ with sigmoid function $\sigma(\cdot)$.  


\subsection{Object detection}
Object detection comprises predicting the location $b\in [0,1]^4$ and scoring for each category $y \in \mathcal{Y}$ of an object that appears in an input image where multiple objects may appear at the same time. In order to predict the location of an object, an object detector will generate a large number of object proposals by sliding through every spatial coordinate of the image and predict a score of whether or not an object is present in the particular location. During training, a few set of confident and spatially diverse set of proposals are selected after filtering process, and a random subset of the remaining proposals are chosen to be background samples. In the probabilistic point of view, we may assume that every image follows a certain prior probability of an object appearance, $\pfg$, such that given a fixed number of total object proposals, $m$, the expected number of objects is $m\cdot \pfg$. Similarly, we can define the prior probability of the mislocalized proposals (background) to be $\pbg = 1-\pfg$. This setting allows us to formulate object detection in entirely probabilistic point of view. 

\subsection{Learning with long-tail data}
We are given training and testing distributions $\pp(x,y)$ and $\qq(x,y)$, where $x\in \mathcal{X}$ an input image (or region of interest) and $y\in \mathcal{Y}$ the corresponding class label. Both distributions are a combination $P(x,y) = P(x|y)P(y)$ of class-distributions $P(y)$ and class-conditional image distributions $P(x|y)$. We assume the training and testing class-conditional image distributions are the same ($\pp(x|y)=\qq(x|y)$) while the class distributions can vary ($\pp(y) \ne \qq(y)$). For common evaluation metrics, the test distribution is usually balanced $\qq(y) = \frac{1}{|\mathcal{Y}|}$ whereas the training distribution $\pp(y)$ is long-tail.


\subsection{Probabilistic AP}
Let us define precision, recall, and average precision (AP) in probabilistic perspective. 
\begin{definition}[Precision]
\begin{align}
\text{Pre}_c( t) 
&= \frac{P_{x\sim \pc}(\sig > t)}{P_{x\sim  \pc}(\sig > t) + \alpha_c  P_{x \sim  \pnc}(\sig > t)}\\
&= \frac{P_{x\sim \pc}(\sig > t)P(y=c)}{P_{x\sim  \pc}(\sig > t)P(y=c) +   P_{x \sim  \pnc}(\sig > t)P(y\ne c)}\\
&= \frac{P_{x, y \sim P(X,Y)}(\sig > t | y=c)P(y=c)}{P_{x,y \sim P(X,Y)}(\sig > t)}\\
&= \underbrace{P_{x, y \sim P(X,Y)}(y=c|\sig > t)}_{\text{``true positive given positive''}}
\end{align}
where $\alpha_c$ is the ratio between negative and positive of class $c$, $\alpha_c = \frac{P(y \ne c)}{P(y=c)}$.
\end{definition}
\begin{definition}[Recall]
\begin{align}
\text{Rec}_c( t) =P_{x\sim  \pc}(\sig > t) = \underbrace{P_{x,y \sim P(X,Y)}(\sig > t | y=c)}_{\text{``positive given true''}}
\end{align}
\end{definition}
\begin{definition}[Average Precision]
\begin{align}
\ap_c 
&= \int^1_0 \pre (\max_{t:\rec(t)<\beta}(t))\mathrm{d}\beta 
\end{align}
\end{definition}
\begin{theorem}
\label{ap_alternative}
Average Precision can be expressed in the following form:
\begin{align}
\ap_c =  \e_{t\sim P_{s_c^+}}[\pre(t)]
\end{align}
\begin{proof}
Let us assume $P_{x\sim \pc}(\f(x)_c)$ is a proper probability distribution. I.e., $P_{x\sim \pc}(\sig)>0$. This means $\max_{t:\rec(t)<\beta}(t)=\rec^{-1}(\beta)$ exists and hence:
\begin{align}
\ap_c 
&= \int^1_0 \pre (\max_{t:\rec(t)<\beta}(t))\mathrm{d}\beta \\
&= \int^1_0 \pre(\rec^{-1}(\beta)) \mathrm{d} \beta \\
&= - \int^{-\infty}_{\infty} \pre(t)\p_{x\sim \pc}(f(x)_c =t) \mathrm{d} t\\
&=  \int^{\infty}_{-\infty} \pre(t)\p_{x\sim \pc}(f(x)_c =t) \mathrm{d} t\\
&= \e_{t\sim P_{s_c^+}}[\pre(t)]
\end{align}
since $\beta =\rec(t) \Longrightarrow \frac{\partial \beta}{\partial t}=\frac{\partial \rec(t)}{\partial t}=-P_{x\sim \pc}(\f(x)_c = t)$, where $P_{s^+_c}$ is the distribution of logits from positive samples. 
\end{proof}
\end{theorem}

\subsection{Pairwise Ranking Error}
Let us introduce a new metric, we call Pairwise Ranking Error (R) for a class $c \in \y$. 
\begin{definition}[Pairwise Ranking Error]
\begin{align}
\pr_c = \p_{x^+, x^- \sim \pc \times \pnc} \big(\sigp < \sigm \big)
\end{align}
This measures \emph{how much a model mis-ranks given a pair of samples from positive and negative distributions}. 
\end{definition}

\begin{theorem}
\label{r_alternative}
Pairwise Ranking can be expressed in the following form:
\begin{align}
\pr_c = \e_{t \sim P_{s^+_c}}\Big[P_{x \sim  \pnc}\big(\sig > t\big)\Big]
\end{align}
\begin{proof}
Since $\pc$ and $\pnc$ are mutually independent:
\begin{align}
\pr_c &= \p_{x^+, x^- \sim \pc \times \pnc} \big( \sigp < \sigm \big)\\
&= \int^\infty_{-\infty} \p_{x^+, x^- \sim \pc \times \pnc} \big(\sigp =t \land t < \sigm \big)\mathrm{d}t \\
&= \int^\infty_{-\infty} \p_{x^+ \sim \pc} \big( \sigp =t\big) P_{x^-\sim \pnc }( \sigm > t \big)\mathrm{d}t \\
&= \e_{t \sim P_{s^+_c}}\Big[P_{x \sim  \pnc}\big(\sig > t\big)\Big]
\end{align}
\end{proof}
\end{theorem}




==> random_math.tex <==

\rule{11cm}{0.4pt}
\begin{align}
R_c 
&\le E_{x\sim \pc}\left[\I{s_c(x) \le t}\right]+E_{x^\prime\sim \pnc}\left[\I{t < s_c(x^\prime)}\right]\\
&=E_{x\sim \pc}\left[\I{s_c(x) \le t}\right]+E_{x^\prime\sim \pnc}\left[\I{1-t > s_{\lnot c}(x^\prime)}\right]
\end{align}
The above is in fact directly applicable with LDAM's binary optimal solution~\cite{ldam}, where in our case the maximum margin ($\beta$) is bounded by $1$, and the solution $t_c^* = \frac{1 \cdot n_{\lnot c}^{1/4}}{n_{ c}^{1/4} + n_{\lnot c}^{1/4}}$ and $t_{\lnot c}^* = \frac{1\cdot n_{ c}^{1/4}}{n_{ c}^{1/4} + n_{\lnot c}^{1/4}}$. Suppose the optimal $t$ from the above optimization is $g^*$. Then, 
\begin{align}
\mathcal{L}^{\text{Det}}_c 
&\lesssim m_c (P_{x\sim D_{c}}(s_{c}(x) < g^*) + P_{x\sim D_{\lnot c}}(s_{c}(x) \ge g^*)\\
&=m_c (P_{x\sim D_{c}}(s_{c}(x) < g^*) + P_{x\sim D_{\lnot c}}(1-s_{c}(x) < 1-g^*)\\
&=m_c (P_{x\sim D_{c}}(\log s_{c}(x) < \log( g^*)) + P_{x\sim D_{\lnot c}}(\log (1-s_{c}(x)) < \log (1-g^*))\\
&=m_c (P_{x\sim D_{c}}(-\log (s_{c}(x)\cdot (g^*)^{-1}) > 0)\\
&+ P_{x\sim D_{\lnot c}}(-\log ((1-s_{c}(x))*(1-g^*)^{-1}) > 0))
\end{align}

And here the upper-bound is minimized as $-\log (s_{c}(x)\cdot (g^*)^{-1})$ for $x\sim D_c$ and $-\log ((1-s_{c}(x))*(1-g^*)^{-1})$ for $x\sim D_{\lnot c}$ reach the minimum. Hence, we can define a surrogate task for a sample $x,y \sim D$:
\begin{align}
\ell_c(x,y) 
&= -m_c  \Big( 1_{[y=c]} \log ((s_{c}(x) \underbrace{(g^*)^{-1}}_{w^+_c})) + 1_{[y\ne c]} \log ((1-s_{c}(x))*\underbrace{(1-g^*)^{-1}}_{w^-_c})
\end{align}
Since we train the detector for all classes in $C$ simultaneously
\begin{align}
\Longrightarrow 
\ell(x,y) 
&= \sum_{c\in C} -m_c  \Big( 1_{[y=c]} \log (s_{c}(x) \cdot  w^+_c) + 1_{[y\ne c]} \log ((1-s_{c}(x)) \cdot w^-_c)\Big)
\end{align}
After normalizing the confidence such that loss will always be non-negative:
\begin{align}
l_{\text{ECM}}(x,y) 
&= - \sum_{c\in C} m_c \Big(1_{[y=c]}\cdot \log (s_{w_c}(x)_c) + 1_{[y\ne c]}\cdot \log (1-s_{w_c}(x)_c) \Big)\\
&= BCE(s_{w_c}(x), y)\\
\text{where}\quad s_{w_c}(x)_c &= \frac{{w_c}^+ \cdot e^{f(x)_c}}{{w_c}^+\cdot e^{f(x)_c} + {w_c}^-\cdot e^{-f(x)_c}}\in [0, 1]\\
\text{and}\quad 1- s_{w_c}(x)_c &= \frac{{w_c}^- \cdot e^{-f(x)_c}}{{w_c}^+\cdot e^{f(x)_c} + {w_c}^-\cdot e^{-f(x)_c}}\in [0, 1]\\
\Longrightarrow s_{w_c}(x)_c 
&= \sigma(2f(x)_c + \log (w^+_c) - \log (w^-_c))\\
&= \sigma(2f(x)_c + \underbrace{1/4\log (n_c) - 1/4\log (n_{\lnot c}}_{\Delta_c}))
\end{align}
Hence, we effectively apply a fixed margin $\Delta_c$ for each class $c\in C$, which we call effective class-margin.

\rule{11cm}{0.4pt}
% Since $s = \sigma \circ f$:

% $$
% \mathcal{L}_c(f) = P_{x\sim D_c}(\sigma(f(x)_c) < \sigma(0))=P_{x\sim D_c}(\sigma(f(x)_c) < \frac{1}{2}) \le P_{x\sim D_c}(\sigma(f(x)_c) < \frac{1}{2} + \gamma_c)\le \hat{\mathcal{L}}_{\gamma_c, c}(f) + \frac{4}{\gamma_c}\sqrt{\frac{C(F)}{n_c}}+\epsilon(n_c)
% $$










==> related.tex <==

\section{Related works}

\paragraph{\textbf{Object detection}} Object detection is largely divided into one-stage and two-stage pipelines. In one-stage object detection~\cite{centernet,focal,yolo,yolov2,yolov3}, classification and localization are simultaneously predicted densely on each coordinate of feature map representation. Hence, one-stage detection faces extreme foreground-background imbalance aside from cross-category imbalance. These issues are addressed either by carefully engineered loss function (e.g., Focal Loss~\cite{focal}), sampling heuristics (e.g., ATSS~\cite{atss}), or implicit anchor assignment to cascade proposals (e.g., CenterNet~\cite{centernet}). In two-stage object detection~\cite{fastrcnn,fasterrcnn,cascadercnn}, fewer number of object proposals are first selected either by cascading via small network (e.g., RPN~\cite{fasterrcnn}) or sampling heuristics. The two-stage detectors tend to have higher accuracy compared to the one-stage counterparts as cascading improves precision and object localization, but one-stage detectors have much faster inference time. For the balanced small-scale dataset such as COCO~\cite{coco}, the choice of detectors is based on the task and trade-off between accuracy and the speed. 


\subsection{Long-tailed Detection} Despite many recent success in alleviating the extreme foreground and background imbalance, learning under severe long-tailed distribution is still challenging. There are different approaches to solve the problem such as by leveraging external dataset~\cite{mosaic}, extensive data augmentation and large backbone~\cite{copypaste}, optimized data-sampling strategies~\cite{lvis,simcal,forest}, and re-weighted loss functions~\cite{eqlv1,eqlv2,seesaw,federated_loss,bags,disalign,deconfound}. In particular to designing loss function, it can be largely categorized into 1) \textbf{explicit} re-weighting and 2) \textbf{implicit} re-weighting. Equalization Loss~\cite{eqlv1} ignores negative gradient for rare classes with the observation that rare classes get {discouraged} with higher frequency of negative gradients. Balanced Group Softmax~\cite{bags} first divides classes into several {groups} by their frequency in training dataset, and applies softmax only within each group. This implicitly controls the negative gradient to the rare classes from frequent classes and background. Federated Loss~\cite{federated} simply ignores negative gradient to classes that have not been appeared within the image, which also implicitly reduces the impact of negative gradient to the rare classes at expectation. On the other hand, EQL v2~\cite{eqlv2} aims to directly balance the ratio of cumulative positive and negative gradients per-class. Seesaw Loss~\cite{seesaw} takes the similar intuition and use class frequency to directly weaken the weight of negative gradients for rare classes as well as to compensate for diminished gradient from any mis-classification by scaling up by the ratio of predicted probability of a class and that of the ground truth class. These methods share the common premise that overwhelming negative gradients will influence the training dynamics of the detector and result biased classifier. All of these methods lack analytical reason that their particular re-weighting schemes should work well. However, interestingly, all these methods can be re-formulated to \textbf{weighted softmax/sigmoid} with different strategies of weight assignment. 


\subsection{Learning with class-margins} Margin-based learning has been widely used in various topics such as face recognition~\cite{large_margin_loss,additive_margin_loss,arcface} as well as classification under imbalanced data~\cite{ldam}. In fact, assigning proper margins has a long history related to generalization error bound~\cite{kakade,lipschitz,barlett,pachenko}. The overall focus is to closely approximate the model's complexity measure $C(\Theta)$ with respect to the number of samples $n$ and objective-specific parameter $\gamma$ (e.g., margin), and bound the test error:
\begin{align}
    \text{Test Error} \lesssim \frac{1}{\gamma} \cdot \sqrt{\frac{C(\Theta)}{n}}
\end{align}
Recently, Cao et al.~\cite{ldam} showed the effectiveness of analytically derived margins for such settings in imbalanced classification task. In \textbf{separable} setting (i.e., training error can converge to 0) for two-class classification, class-margins can be derived by simple constrained optimization. Since many recent methods in long-tail object detection can be reformulated into re-weighted loss (or equivalently, soft-margin loss), we motivate the need to approach the problem in the perspective of margin theory. However, object detection has fundamentally different evaluation metric, AP. In AP, distribution of model's confidence and data distribution is deeply intertwined in the form of precision and recall, and it is unclear how to relate the metric to the long-studied margin-based learning. 


==> result.tex <==
\section{Experiments}

\input{table_1x}
\input{table_main}
\input{table_1stage_1x}
\input{table_oid}

\subsection{Experimental Settings}
\myparagraph{Datasets.} Our method is tested mainly on LVIS v1.0~\cite{lvis} dataset. LVIS v1.0 is a large-scale object detection and instance segmentation dataset, with includes 1203 object categories which follows extreme long-tail distribution. Object categories in LVIS dataset are divided into three groups by frequency: \textit{frequent}, \textit{common}, and \textit{rare}. Categories that appear on less than 10 images is considered rare, more than 10 but less than 100 is common, and frequent otherwise. There are about 1.3 M instances in the dataset over 120k images (100k train, 20k validation split). Additionally, we test our method on OpenImages Object Detection dataset, another large-scale dataset with 500 object categories over 1.7 M images, with similar degree of long-tail nature. 

\myparagraph{Evaluation. } We test the models trained with ECM Loss and other methods on both the conventional evaluation metric ($\text{mAP}$) as well as the newly proposed metric ($\text{mAP}_{\text{fixed}}$~\cite{ap_fixed}). $\text{mAP}$ measures the mean average precision over IoU thresholds from 0.5 to 0.95 similar to~\cite{coco}, but for each image the number of detection is extended to 300.  $\text{mAP}_{\text{fixed}}$~\cite{ap_fixed} improves the original metric by setting no limit for per-image detection but instead setting 10k per-\textit{class} detection predictions over the entire dataset. Please note that due to exploding memory consumption of mask prediction, we limit per-image detection to 800 instead of $\infty$. We also evaluate based on the boundary IoU ($\text{mAP}_{\text{boundary}}$~\cite{boundary_iou}), which is also the new evaluation metric in this year's LVIS Challenge.
For OpenImages, we follow evaluation protocol of~\cite{unidet} and measure mAP@0.5.

% As seen in Table {\ref{tab:maskr50_result}}, \ours consistently makes substantial gain over other methods, showing that the derived effective class-margins are not over-fitted to a particular evaluation metric.
% We additionally test our method on OpenImages~\cite{openimages} to show generality. 

\subsection{Implementation Details.} 
Our implementation is based on Detectron2~\cite{detectron2} and MMDetection~\cite{mmdet}, two most popular open-source libraries for object detection tasks. Below, we will explain details of implementation for two-stage and one-stage detectors.

\myparagraph{Two-stage benchmark.} For two-stage, we train instance segmentation models. We test our method on Mask R-CNN~\cite{maskrcnn} and Cascade Mask R-CNN~\cite{cascadercnn} with various backbones, ResNet-50 and ResNet-101~\cite{resnet} with Feature Pyramid Network~\cite{fpn} pretrained on ImageNet-1K~\cite{imagenet}. Additionally, we also test on recently successful Transformer-based backbone Swin Transformer~\cite{swin} pretrained on ImageNet-21K with 224x224 image resolution. We train with for 12 and 24 epochs (1x and 2x schedules, respectively), with Repeated Factor Sampler (RFS)~\cite{lvis}. 
For the models with CNN-based backbones, we use SGD optimizer with 0.9 momentum, initial learning rate of 0.02, weight decay of 0.0001, with step-wise scheduler decaying learning rate by 0.1 after 20 and 22 epochs, and batch size of 16 on 8 GPUs.  For Transformer-based backbones, we use AdamW optimizer with initial learning rate of $0.00005$, beta set to $(0.9, 0.999)$, weight decay of $0.05$, with Cosine-annealing scheduler. For all our models, we follow the standard data augmentation during training: random horiziontal flipping and multi-scale image resizing to fit the shorter side of image to ($640, 672, 704, 736, 768, 800$) at random, and the longer side kept smaller than $1333$. For Swin Transformer, we use larger range of scale of the short side of image from $480$ to $800$. For two-stage detectors, we normalize the classification layers with temperature $\tau=20$ for both box and mask classifications, and apply foreground calibration as post-process following prior practices~\cite{seesaw,disalign,ap_fixed}. Since in LVIS there are more number of instances than COCO, we increased per-image detection limit to 300 from 100 and set the confidence threshold to 0.0001 as a common practice~\cite{lvis}. For OpenImages experiment, we train Cascade R-CNN with ResNet-50 backbone following the baseline from~\cite{unidet}. All models in this experiment were trained for 180k iterations with Class-aware Sampler, closely following the training and evaluation protocol of~\cite{unidet}.  


\myparagraph{One-stage benchmark.} We further test our method on one-stage detectors. For one-stage detectors, Focal Loss~\cite{focal} is a standard choice of loss function, which effectively diminishes loss values for ``easy'' samples such as background. In this experiment, we test compatibility of our method with Focal weights. More specifically, we simply apply the computed focal weights on ECM Loss, which is a binary cross-entropy with the weighted sigmoid function (surrogate scoring function $\hat{s}$). We test our ECM Loss with focal weight on a number of popular one-stage detectors: FCOS~\cite{fcos}, ATSS~\cite{atss} and VarifocalNet~\cite{varifocal}. Each method uses either Focal Loss or a variant such as Varifocal Loss~\cite{varifocal}. We use the default hyperparameter for all types of focal weights: $\gamma=2, \alpha=0.25$ for Focal Loss, $\gamma=2$ and $\alpha=0.75$ for Varifocal Loss. Since in LVIS v1.0 models expect to see more instances, we double the per-pyramid level number of anchor candidates from $9$ to $18$ for ATSS and VarifocalNet. Similar to 2-stage detectors, we increased per-image detection to 300 and set the confidence threshold to 0.0001. We train on ResNet-50 and ResNet-101 backbones for 12 epochs, batch size of 16 on 8 GPUs. We set the learning rate to be 0.01 which was the optimal learning rate for the baselines. 

\myparagraph{ECM Loss.} Our ECM Loss is extremely simplistic and easy to plug-in to any form of detectors. Notably, ECM Loss does not require any hyper-parameter. We use available annotation set from each dataset to measure the training prior distribution of each class. Note that in object detector, background probability is ill-defined, as each detector may have different internal mechanism to gather the regions of interest and hence the background probability for different detectors may differ slightly. We empirically measured the frequency of background samples in the \textit{classification layer} during the first few iterations. Then, we compute the class frequency \textit{with background} and use it to compute the effective class-margins. For one-stage detectors, we only count for foreground classes as foreground and background imbalance is managed from focal weight~\cite{focal}. 

\subsection{Experimental Results}
In this section, we will discuss about the experimental results of our method. 

\myparagraph{Two-stage detection.} In Table~\ref{tab:table_1x} and Table~\ref{tab:table_main}, we compare our approach with other methods. In Table~\ref{tab:table_1x}, we compare methods on Mask R-CNN with ResNet-50 backbone on 1x schedule. Our ECM Loss achieves 26.3 $\text{mAP}_{\text{segm}}$ and 26.7 $\text{mAP}_{\text{bbox}}$, which is 1.1 and 1.3 points higher than the state-of-the-art performance on the same configuration. Notably, our method achieves \textbf{10} points gain over cross-entropy loss baseline as well as \textbf{3.1} point gain over the state of the art performance on $\text{AP}_{\text{r}}$. Moreover, our method shows similar gains on the new evaluation metrics $\text{mAP}^{\text{fixed}}_{\text{boundary}}$ and $\text{mAP}^{\text{fixed}}_{\text{bbox}}$ whereas other methods tend to diminish the gains from the old metrics. Note that our method requires 0 hyperparameter while other competitive methods do. 

In Table~\ref{tab:table_main}, we extend the experiment scale and evaluate with various frameworks and backbones, on longer 2x training schedule. With Mask R-CNN with ResNet-50 backbone, ECM Loss achieves 27.4 $\text{mAP}_{\text{segm}}$ and 27.9 $\text{mAP}_{\text{bbox}}$, and with ResNet-101 backbone, it achieves 28.7 $\text{mAP}_{\text{segm}}$ and 29.4 $\text{mAP}_{\text{bbox}}$. With more advanced Cascade R-CNN framework, ECM Loss achives 30.6 and 33.4 points, respectively. Finally, with the recent Swin-B backbone pre-trained on ImageNet-21k, ECM Loss outperforms Seesaw Loss with 39.7 and 43.6 points, respectively. For all choice of framework and backbone, our method consistently outperforms the state-of-the-art performances. Please note that Seesaw Loss~\cite{seesaw} has been applied to the first-place winner solutions of LVIS challenge 2020 and 2021. 

In Table~\ref{tab:table_oid}, we compare ECM Loss with a variant of Equalization Loss with class hierarchy from~\cite{unidet}. Although OpenImages have long-tail distribution of classes, the number of classes and the associated prior probabilities are very different. Nevertheless, ECM Loss improves over the baseline for 0.9 mAP, which is comparable to the same baseline trained for 8x schedule. This result confirms generality of our method. 


\myparagraph{One-stage detection.} In Table~\ref{tab:table_1stage_1x}, FCOS, ATSS and VarifocalNet are used to compare ECM Loss over baseline losses, trained with ResNet-50 and ResNet-101 backbones on 1x schedule. As seen in Table~\ref{tab:table_1stage_1x}, ECM Loss has consistent gain over Focal Loss and its variants. With FCOS, ECM improves box mAP 1.2 and 1.1 points, respectively, for ResNet-50 and ResNet-101 backbones. With ATSS, ECM Loss improves Focal Loss \textbf{7.2} and \textbf{4.8} points on $\text{AP}_{\text{r}}$, and \textbf{2.4} and \textbf{1.3} points mAP, respectively. We further test on VarifocalNet, recently proposed one-stage detector and show similar advantage on ResNet-50 backbone. In sum, we confirm that our ECM Loss consistently improves overall score on one-stage detectors especially on rare classes. 

\section{Conclusion}
In this paper, we tackle long-tail object detection problem in a statistical approach. We connect the training objective and the detection evaluation objective in the form of margin theory. We first relax the average precision computation into a ranking err with monotonic upper and lower bounds, and simplify by approximating on a linear line. Then, we further reduce the ranking err into a specific form of binary classification error with provably optimal class-margins. From this, we introduced our Effective Class-Margin Loss, a form of binary cross-entropy loss with our surrogate scoring function with the class-margins. We verify the advantage of our loss function in multiple perspectives; ECM Loss is simple and requires no hyperparameters, outperforms state-of-the-arts on various frameworks and backbones, and general to be applicable in one-stage detection pipeline as well as two-stage detection.   

==> table_new.tex <==
\newcommand{\n}{5}

\begin{table*}
\begin{center}
\caption{Comparison on LVIS v1 validation set with new evaluation metric. Models are trained with Mask R-CNN with ResNet-50 backbone on 1x schedule.  }
\label{tab:maskr50_result}
\resizebox{0.65\linewidth}{!}{
\begin{tabular}{lccccc}
 Method  & $\text{mAP}_{\text{segm}}$ & $\text{AP}_{\text{r}}$ & $\text{AP}_{\text{c}}$& $\text{AP}_{\text{f}}$ & $\text{mAP}_{\text{bbox}}$  \\
\toprule
RFS+CE Loss &\\
BAGS~\cite{bags} & \\
EQL v2~\cite{eqlv2} & \\ 
Federated Loss~\cite{federated_loss}  &\\
DisAlign~\cite{disalign} & \\
Seesaw Loss~\cite{seesaw}  &\\
RFS+RS Loss~\cite{ranksort} & \\
\midrule
\ours& \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table*}


==> teaser.tex <==
\begin{figure}[t]
\begin{center}
% \begin{overpic} 
% [width=\linewidth]
% {example-image-a}
% \end{overpic}
\includegraphics[width=0.5\linewidth]{teaser.png}
\end{center}
\caption{
% 
Assigning class-margins affect the training dynamics of a neural network. We show that there exists \textbf{effective class-margins} that leads to better performance when training under long-tailed data distribution. }
\label{fig:teaser}
\end{figure}
